Unlocking the Potential of Model Calibration in Federated Learning

Over the past several years, various federated learning (FL) methodologies have been developed to improve model accuracy, a primary performance metric in machine learning. However, to utilize FL in practical decision-making scenarios, beyond considering accuracy, the trained model must also have a reliable confidence in each of its predictions, an aspect that has been largely overlooked in existing FL research. Motivated by this gap, we propose Non-Uniform Calibration for Federated Learning (NUCFL), a generic framework that integrates FL with the concept of model calibration. The inherent data heterogeneity in FL environments makes model calibration particularly difficult, as it must ensure reliability across diverse data distributions and client conditions. Our NUCFL addresses this challenge by dynamically adjusting the model calibration objectives based on statistical relationships between each client's local model and the global model in FL. In particular, NUCFL assesses the similarity between local and global model relationships, and controls the penalty term for the calibration loss during client-side local training. By doing so, NUCFL effectively aligns calibration needs for the global model in heterogeneous FL settings while not sacrificing accuracy. Extensive experiments show that NUCFL offers flexibility and effectiveness across various FL algorithms, enhancing accuracy as well as model calibration.

==> table/CIFAR100_nonIID05.tex <==

\begin{table*}
\small
\begin{center}
\scalebox{0.44}{
\begin{tabular}{c||ccc|ccc|ccc|ccc|ccc}
\hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {\textbf{Calibration}} \\ {\textbf{Method}}\end{tabular}}  & \multicolumn{3}{c|}{\textbf{FedAvg}} & \multicolumn{3}{c|}{\textbf{FedProx}}  & \multicolumn{3}{c|}{\textbf{Scaffold}} & \multicolumn{3}{c|}{\textbf{FedDyn}} & \multicolumn{3}{c}{\textbf{FedNova}}\\
  & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$ & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$  & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$ & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$ & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$\\
\hline\hline
Uncal. & 61.34 $\pm$ 1.31	 & 10.52 $\pm$ 1.17 & 3.61  $\pm$ 0.93 & 61.88 $\pm$ 1.55	 & 9.37 $\pm$ 1.21 & 3.58  $\pm$ 1.05 & 62.08 $\pm$ 0.97	 & 11.42 $\pm$ 2.05 & 3.82  $\pm$ 1.55 & 62.39 $\pm$ 1.25	 & 12.53 $\pm$ 1.25 & 3.84  $\pm$ 1.10 & 63.01 $\pm$ 1.62	 & 11.45 $\pm$ 1.05 & 3.82  $\pm$ 0.79
\\
Focal& 60.59 $\pm$ 1.42	 & 12.88 $\pm$ 0.95 & 3.74  $\pm$ 1.35 & 62.07 $\pm$ 1.39	 & 11.45 $\pm$ 1.04 & 3.79  $\pm$ 0.91 & 61.39 $\pm$ 1.15	 & 13.28 $\pm$ 1.71 & 4.88  $\pm$ 1.30 & 60.21 $\pm$ 1.04	 & 11.22 $\pm$ 1.00 & 3.81  $\pm$ 0.95 & 61.15 $\pm$ 1.82	 & 13.21 $\pm$ 1.34 & 4.71  $\pm$ 1.06
\\
LS  & 59.35 $\pm$ 2.15	 & 15.61 $\pm$ 1.27 & 6.28 $\pm$ 1.74 & 62.23 $\pm$ 1.48	 & 14.37 $\pm$ 1.35 & 6.14  $\pm$ 1.55 & 62.15 $\pm$ 1.53	 & 11.69 $\pm$ 1.84 & 4.05  $\pm$ 1.07& 61.34 $\pm$ 1.45	 & 15.19 $\pm$ 2.08 & 6.58  $\pm$ 1.54 & 63.05 $\pm$ 2.25	 & 16.03 $\pm$ 2.00 & 6.89  $\pm$ 1.85
\\
BS  & 61.20 $\pm$ 1.95	 & 11.32 $\pm$ 1.44 & 3.80 $\pm$ 1.10 & 60.43 $\pm$ 1.04	 & 10.15 $\pm$ 1.38 & 3.61  $\pm$ 1.17 & 60.39 $\pm$ 1.30	 & 10.92 $\pm$ 1.33 & 3.80  $\pm$ 1.10  & 62.17 $\pm$ 1.42	 & 13.81 $\pm$ 1.27 & 4.91  $\pm$ 0.91 & 60.44  $\pm$ 1.04	 & 11.39 $\pm$ 1.61 & 4.06  $\pm$ 1.24
\\

MMCE  &  60.00 $\pm$ 1.07	 & 13.41 $\pm$ 2.05 & 4.93 $\pm$ 1.72 & 60.11 $\pm$ 1.25	 & 11.32 $\pm$ 1.22 & 3.77  $\pm$ 1.39  & 61.03 $\pm$ 1.22	 & 11.37 $\pm$ 1.52 & 3.83  $\pm$ 1.08 & 61.35 $\pm$ 1.07	 & 12.93 $\pm$ 1.35 & 3.95 $\pm$ 1.11  & 61.28  $\pm$ 1.33	 & 12.55 $\pm$ 1.40 & 3.90  $\pm$ 1.09
\\

FLSD &  58.71 $\pm$ 2.59 & 11.51 $\pm$ 1.33 & 3.92 $\pm$ 1.05 &  59.28 $\pm$ 1.49	 & 10.66 $\pm$ 1.39 & 3.81  $\pm$ 1.04 & 60.49 $\pm$ 1.35	 & 13.61 $\pm$ 1.51 & 5.15  $\pm$ 0.99 & 60.94 $\pm$ 2.11	 & 11.83 $\pm$ 1.04 & 4.04 $\pm$ 0.91 & 60.49  $\pm$ 1.52	 & 13.81 $\pm$ 1.23 & 4.88  $\pm$ 0.99
\\
MbLS  & 59.62 $\pm$ 2.31 & 9.42 $\pm$ 1.58 & 3.55 $\pm$ 0.96 & 60.39 $\pm$ 1.11	 & 11.37 $\pm$ 1.90 & 3.84  $\pm$ 1.25 & 61.389 $\pm$ 1.67	 & 11.99 $\pm$ 1.93 & 4.07  $\pm$ 1.25  & 62.30 $\pm$ 1.51	 & 14.95 $\pm$ 1.41 & 6.50 $\pm$ 1.22 & 62.93  $\pm$ 1.95	 & 13.66 $\pm$ 1.64 & 4.69  $\pm$ 1.04
\\


\hline
DCA & 61.24 $\pm$ 1.20 & 7.69 $\pm$ 1.11 & 3.24 $\pm$ 1.03 & 61.93 $\pm$ 1.17 & 8.74 $\pm$ 1.22 & 3.40  $\pm$ 0.93 & 62.11 $\pm$ 1.20	 & 9.25 $\pm$ 1.32 & 3.55  $\pm$ 0.88 & 62.93 $\pm$ 1.04	 & 10.17 $\pm$ 1.04 & 3.75  $\pm$ 0.92  & 63.15 $\pm$ 1.38	 & 9.27 $\pm$ 0.94 & 3.55  $\pm$ 0.61
\\

\textbf{NUCFL} (DCA+COS) &  61.88 $\pm$ 1.05 & 6.21 $\pm$ 0.95 & 3.11 $\pm$ 0.84 & 62.38 $\pm$ 1.04 & 8.15 $\pm$ 1.01 & 3.35  $\pm$ 0.77 & 62.17 $\pm$ 1.06 & 8.88 $\pm$ 1.04 & 3.50  $\pm$ 0.79 & 62.81 $\pm$ 0.91 & 9.29 $\pm$ 0.95 & 3.54  $\pm$ 0.67 & 63.24 $\pm$ 1.29	 & 8.85 $\pm$ 1.11 & 3.51  $\pm$ 0.82
\\
\textbf{NUCFL}  (DCA+L-CKA) &  62.05 $\pm$ 1.17 & \underline{\textbf{6.14}} $\pm$ 1.03 & \underline{\textbf{3.07}} $\pm$ 0.95 & 62.31 $\pm$ 1.21 & \textbf{8.04} $\pm$ 1.19 & \textbf{3.30}  $\pm$ 0.95 & 62.25 $\pm$ 1.14 & \textbf{8.41} $\pm$ 1.15 & \textbf{3.45}  $\pm$ 1.00  & 62.94 $\pm$ 1.22 & \underline{\textbf{9.14}} $\pm$ 1.22 & \underline{\textbf{3.52}}  $\pm$ 0.84 & 63.27 $\pm$ 1.30	 & 8.52 $\pm$ 0.94 & 3.43  $\pm$ 0.64
\\
\textbf{NUCFL}  (DCA+RBF-CKA) & 61.59 $\pm$ 0.95 & 6.19 $\pm$ 1.22 & 3.11 $\pm$ 1.13 & 61.89 $\pm$ 1.10 & 8.17 $\pm$ 1.04 & 3.35  $\pm$ 0.73 & 61.94 $\pm$ 0.92 & 8.52 $\pm$ 2.00 & \textbf{3.45}  $\pm$ 1.33 & 62.84 $\pm$ 1.15 & 9.21 $\pm$ 1.04 & 3.55  $\pm$ 0.92 & 63.17 $\pm$ 1.17	 & \underline{\textbf{8.01}} $\pm$ 1.08 & \underline{\textbf{3.30}}  $\pm$ 0.85
\\


\hline
MDCA & 61.03 $\pm$ 1.31 & 7.71 $\pm$ 1.50 & 3.29 $\pm$ 1.19  & 62.00 $\pm$ 1.73	 & 8.21 $\pm$ 1.45 & 3.37  $\pm$ 1.10 & 62.23 $\pm$ 1.10	 & 9.04 $\pm$ 1.29 & 3.51  $\pm$ 1.00  & 62.84 $\pm$ 0.82	 & 10.24 $\pm$ 0.85 & 3.72  $\pm$ 0.59 & 63.29 $\pm$ 1.06	 & 10.00 $\pm$ 1.15 & 3.71  $\pm$ 0.74
\\
 
\textbf{NUCFL}  (MDCA+COS) & 62.00 $\pm$ 1.33 & 6.38 $\pm$ 1.07 & 3.14 $\pm$ 0.98  & 61.93 $\pm$ 1.34	 & 7.94 $\pm$ 1.29 & 3.29  $\pm$ 1.33 & 62.17 $\pm$ 0.87	 & 8.31 $\pm$ 1.17 & \underline{\textbf{3.40}}  $\pm$ 0.75 & 62.91 $\pm$ 1.04	 & 9.33 $\pm$ 1.02 & 3.56  $\pm$ 0.91& 63.14 $\pm$ 1.11	 & 9.16 $\pm$ 1.24 & 3.58  $\pm$ 0.99
\\
\textbf{NUCFL}  (MDCA+L-CKA) & 62.17 $\pm$ 1.40 & 6.25 $\pm$ 1.43 & 3.11 $\pm$ 1.24 & 62.03 $\pm$ 1.25	 & \underline{\textbf{7.88}} $\pm$ 1.04 & \underline{\textbf{3.25}}  $\pm$ 0.95 & 62.22 $\pm$ 1.04	 & \underline{\textbf{8.30}} $\pm$ 1.25 & \underline{\textbf{3.40}}  $\pm$ 0.95 & 62.88 $\pm$ 0.95	 & \textbf{9.19} $\pm$ 0.84 & \textbf{3.53}  $\pm$ 0.62 & 63.14 $\pm$ 1.51	 & 9.03 $\pm$ 1.48 & 3.51  $\pm$ 1.17
\\
\textbf{NUCFL}  (MDCA+RBF-CKA) & 61.54 $\pm$ 1.08 & \textbf{6.20} $\pm$ 1.66 & \textbf{3.09} $\pm$ 1.39 & 61.79 $\pm$ 1.04	 & 8.02 $\pm$ 1.38 & 3.29  $\pm$ 1.07 & 62.15 $\pm$ 1.22	 & 8.42 $\pm$ 1.03 & 3.45  $\pm$ 1.11  & 62.65 $\pm$ 1.12	 & 9.24 $\pm$ 1.20 & 3.55  $\pm$ 0.94  & 63.22 $\pm$ 1.35	 & \textbf{8.59} $\pm$ 1.27 & \textbf{3.47}  $\pm$ 1.06
\\


\hline

\end{tabular}
}
\caption{\small Accuracy (\%), calibration measures ECE (\%), and SCE (\%) of various federated optimization methods with different calibration methods under non-IID ($\alpha = 0.5$) scenario on the CIFAR-100 dataset. Underlined values 
%in boldface 
indicate the best calibration across all methods.}
\vspace{-3mm}
\label{tb:cifar100_noniid05}
\end{center}
\end{table*}


==> table/CIFAR100_resnet_alldistribution.tex <==

\begin{table*}
\small
\begin{center}
\scalebox{0.485}{
\begin{tabular}{c||ccc|ccc|ccc|ccc}
\hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} {\textbf{Calibration}} \\ {\textbf{Method}}\end{tabular}}  & \multicolumn{3}{c|}{\textbf{IID}} & \multicolumn{3}{c|}{\textbf{Non-IID ($\alpha = 0.5$)}}  & \multicolumn{3}{c|}{\textbf{Non-IID ($\alpha = 0.1$)}} & \multicolumn{3}{c}{\textbf{Non-IID ($\alpha = 0.05$)}}\\
  & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$ & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$  & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$ & {Acc} $\uparrow$ & {ECE} $\downarrow$ & {SCE} $\downarrow$\\
\hline\hline
Uncal. &  65.19 $\pm$ 1.25	 & 7.61 $\pm$ 1.04 & 3.25  $\pm$ 0.89 & 61.34 $\pm$ 1.31	 & 10.52 $\pm$ 1.17 & 3.61  $\pm$ 0.93 & 58.34 $\pm$ 1.66	 & 12.02 $\pm$ 1.39 & 3.80  $\pm$ 0.97 & 56.77 $\pm$ 1.42 & 14.80 $\pm$ 0.91 & 4.77 $\pm$ 0.51\\

Focal& 63.88 $\pm$ 1.61	 & 11.21 $\pm$ 1.32 & 3.78  $\pm$ 1.09 &  60.59 $\pm$ 1.42	 & 12.88 $\pm$ 0.95 & 3.74  $\pm$ 1.35 & 57.59 $\pm$ 1.13 & 14.28 $\pm$ 1.20 & 4.60  $\pm$ 1.22 & 55.61 $\pm$ 1.18 & 15.96 $\pm$ 0.84 & 5.20 $\pm$ 0.56
\\
LS  & 63.17 $\pm$ 1.67	 & 12.19 $\pm$ 1.08 & 3.88 $\pm$ 0.94 & 59.35 $\pm$ 2.15	 & 15.61 $\pm$ 1.27 & 6.28 $\pm$ 1.74 & 56.35 $\pm$ 2.42 & 12.01 $\pm$ 1.54 & 3.81 $\pm$ 1.95 & 56.26 $\pm$ 1.45 & 14.59 $\pm$ 0.98 & 4.71 $\pm$ 0.60 
\\
BS  &65.00 $\pm$ 1.71	 & 8.51 $\pm$ 1.24 & 3.38 $\pm$ 1.00 & 61.20 $\pm$ 1.95	 & 11.32 $\pm$ 1.44 & 3.80 $\pm$ 1.10 & 56.20 $\pm$ 2.19 & 11.72 $\pm$ 1.66 & 4.20 $\pm$ 1.24 & 55.26 $\pm$ 1.56 & 13.98 $\pm$ 0.92 & 4.72 $\pm$ 0.49 \\

MMCE  &  65.03 $\pm$ 1.61	 & 10.01 $\pm$ 1.20 & 3.73 $\pm$ 1.01 & 60.00 $\pm$ 1.07	 & 13.41 $\pm$ 2.05 & 4.93 $\pm$ 1.72 & 57.00 $\pm$ 1.34 & 11.81 $\pm$ 2.29 & 3.83 $\pm$ 1.00 & 57.64 $\pm$ 1.29 & 16.66 $\pm$ 0.95 & 3.87 $\pm$ 0.57
\\

FLSD & 63.11 $\pm$ 1.37 & 8.15 $\pm$ 1.04 & 3.36 $\pm$ 0.50 &  58.71 $\pm$ 2.59 & 11.51 $\pm$ 1.33 & 3.92 $\pm$ 1.05 & 58.71 $\pm$ 1.85 & 11.91 $\pm$ 1.52 & 3.77 $\pm$ 1.14 & 54.10 $\pm$ 1.35 & 11.29 $\pm$ 0.89 & 3.56 $\pm$ 0.51 
\\
MbLS  &  64.17 $\pm$ 1.95 & 8.60 $\pm$ 1.64 & 3.47 $\pm$ 1.41 &  59.62 $\pm$ 2.31 & 9.42 $\pm$ 1.58 & 3.55 $\pm$ 0.96 &  58.62 $\pm$ 1.49 & 13.82 $\pm$ 1.82 & 4.75 $\pm$ 0.95 & 55.16 $\pm$ 1.55 & 14.99 $\pm$ 1.08 & 4.80 $\pm$ 0.61
\\


\hline
DCA & 65.63 $\pm$ 1.14 & 6.11 $\pm$ 1.05 & 3.06 $\pm$ 0.92&  61.24 $\pm$ 1.20 & 7.69 $\pm$ 1.11 & 3.24 $\pm$ 1.03 & 59.19 $\pm$ 1.12 & 10.45 $\pm$ 0.87 & 3.61 $\pm$ 0.54 &  56.19 $\pm$ 0.98 & 13.05 $\pm$ 0.42 & 3.99 $\pm$ 0.35 
\\

\textbf{NUCFL} (DCA+COS) &  65.66 $\pm$ 1.07 & 6.04 $\pm$ 1.10 &  3.01 $\pm$ 0.85  & 61.88 $\pm$ 1.05 & 6.21 $\pm$ 0.95 & 3.11 $\pm$ 0.84 &  58.97 $\pm$ 1.25 & 9.35 $\pm$ 0.90 & 3.55 $\pm$ 0.65 & 56.97 $\pm$ 1.05 & 11.95 $\pm$ 0.40 & 3.64 $\pm$ 0.33 
\\
\textbf{NUCFL}  (DCA+L-CKA) & 65.43 $\pm$ 1.12 & 5.98 $\pm$ 1.03 &  2.99 $\pm$ 0.78  & 62.05 $\pm$ 1.17 & \underline{\textbf{6.14}} $\pm$ 1.03 & \underline{\textbf{3.07}} $\pm$ 0.95 & 60.73 $\pm$ 1.20 & \underline{\textbf{9.14}} $\pm$ 0.85 & \underline{\textbf{3.50}} $\pm$ 0.45 & 57.03 $\pm$ 1.21 & \underline{\textbf{10.24}} $\pm$ 0.42 & \underline{\textbf{3.52}} $\pm$ 0.11 
\\
\textbf{NUCFL}  (DCA+RBF-CKA) & 65.31 $\pm$ 0.95 & \underline{\textbf{5.94}} $\pm$ 1.13 & \underline{\textbf{2.96}} $\pm$ 0.92  & 61.59 $\pm$ 0.95 & 6.19 $\pm$ 1.22 & 3.11 $\pm$ 1.13 & 59.20 $\pm$ 1.30 & 10.16 $\pm$ 0.94 & 3.60 $\pm$ 0.61 &  56.90 $\pm$ 1.11 & 10.76 $\pm$ 0.39 & 3.54 $\pm$ 0.34
\\


\hline
MDCA & 65.32 $\pm$ 1.25 & 6.25 $\pm$ 1.06 & 3.12 $\pm$ 0.69 & 61.03 $\pm$ 1.31 & 7.71 $\pm$ 1.50 & 3.29 $\pm$ 1.19 & 59.47 $\pm$ 1.22 & 10.19 $\pm$ 1.14 & 3.60 $\pm$ 0.66 & 57.32 $\pm$ 1.01 & 12.79 $\pm$ 0.48 & 3.90 $\pm$ 0.39 
\\
 
\textbf{NUCFL}  (MDCA+COS) & 65.41 $\pm$ 1.04 & 6.17 $\pm$ 1.11 & 3.10 $\pm$ 0.82   & 62.00 $\pm$ 1.33 & 6.38 $\pm$ 1.07 & 3.14 $\pm$ 0.98 & 59.24 $\pm$ 1.15 & 9.74 $\pm$ 0.95 & \textbf{3.59} $\pm$ 0.69 & 56.94 $\pm$ 1.23 & 11.34 $\pm$ 0.42 & \textbf{3.76} $\pm$ 0.33
\\
\textbf{NUCFL}  (MDCA+L-CKA) & 65.50 $\pm$ 1.27 & \textbf{6.04} $\pm$ 1.09 & \textbf{3.02} $\pm$ 0.66 & 62.17 $\pm$ 1.40 & 6.25 $\pm$ 1.43 & 3.11 $\pm$ 1.24 &  59.64 $\pm$ 1.44 & \textbf{9.70} $\pm$ 1.31 &\textbf{3.59} $\pm$ 1.07 & 57.44 $\pm$ 1.33 & \textbf{11.30} $\pm$ 0.41 & \textbf{3.76} $\pm$ 0.29 
\\
\textbf{NUCFL}  (MDCA+RBF-CKA) & 65.44 $\pm$ 1.06 & 6.08 $\pm$ 1.23 & 3.05 $\pm$ 0.92  & 61.54 $\pm$ 1.08 & \textbf{6.20} $\pm$ 1.66 & \textbf{3.09} $\pm$ 1.39 & 58.71 $\pm$ 1.14 & 10.09 $\pm$ 0.89 & 3.61 $\pm$ 0.60 & 56.51 $\pm$ 1.04 & 11.69 $\pm$ 0.46 & 3.82 $\pm$ 0.34 
\\


\hline

\end{tabular}
}
\caption{\small FedAvg all distribution.}
\vspace{-3mm}
\label{tb:cifar100_noniid05}
\end{center}
\end{table*}

